Graph Element Networks: adaptive, structured computation and memory

We explore the use of graph neural networks (GNNs) to model spatial processes in which there is no a priori graphical structure. Similar to finite element analysis, we assign nodes of a GNN to spatial locations and use a computational process defined on the graph to model the relationship between an initial function defined over a space and a resulting function in the same space. We use GNNs as a computational substrate, and show that the locations of the nodes in space as well as their connectivity can be optimized to focus on the most complex parts of the space. Moreover, this representational strategy allows the learned input-output relationship to generalize over the size of the underlying space and run the same model at different levels of precision, trading computation for accuracy. We demonstrate this method on a traditional PDE problem, a physical prediction problem from robotics, and learning to predict scene images from novel viewpoints.

==> dumpster.tex <==

Two other theoretical advantages, which we don't experimentally showcase in this work:
\begin{itemize}
    \item Active memory: propagation in GENs integrates information from multiple sources and allows retrievals at points different than those that were not inputs. An active memory can potentially reduce pressure from an agent which has to integrate memories and act in an environment.
    \item Self-optimizing memory: in the same way we can optimize graphs for better predictions in supervised learning settings, memory GENs could optimize themselves for more efficient retrievals.
\end{itemize}

\section{Graph Element Networks}
\subsection{Abstract Graph Networks} \label{subsec:AGN}
\Add{potentially take out section}
In general, GNNs are applied in settings where nodes and edges are \textit{explicit} and match concrete entities of the domain. For instance, nodes can be objects~\citep{chang2016compositional,battaglia2016interaction}, parts of these objects \citep{wang2018nervenet,mrowca2018flexible} or users in a social network. In general, nodes and edges represent explicit entities and relations, and supervised data is required for each component. We propose to use GNNs as an abstraction of a system's sub-parts,without a concrete match between entities and nodes. 

Let $\gG$ be a graph,% with nodes $n_1,\dots, n_r$ and edges $e_1,\dots,e_{r'}$.
we define an encoding function $f_{in}$ that goes from input to initial states of the nodes and edges in $\gG$. We run several steps of message passing \citep{gilmer2017neural}: in each step, nodes read incoming messages, which are a function of their neighbours' hidden states and their corresponding edges, and use their current state and the sum of incoming messages to compute their new state. 
%We could have used Graph Network blocks \citep{battaglia2018relational} instead at the cost of more complexity. 
Finally, we define a function $f_{out}$ that maps the nodes final states to the final output: $f_{out}\left(MP^{(T)}\left(f_{in}(x)\right)\right)$; trainable end-to-end. This defines a means of combination for the modules, giving us different (differentiable) losses depending on the module we put in each position.
\subsection{Finite Element Methods and Graph Element Networks} \label{subsec:FEM}
\textit{Finite element methods}(FEMs) are a widely used tool in engineering to solve boundary-value problems for partial differential equations. They subdivide a complex problem in a domain (such as analyzing stress forces on a bridge or temperature in a building) into a mesh of small elements where the dynamics of the PDE can be approximated.

With this inspiration, we propose a subtype of abstract graph network, which we denote \textit{graph element network (GEN)}. In GENs, we \textit{place} nodes in a region $\mathcal{R}$ (usually a manifold of $\mathbb{R}^2$ or $\mathbb{R}^3$); each having specific coordinates. In GENs nodes are still abstract (meaning they do not have a 1-to-1 correspondence with a discrete element in the system), but they are \textit{grounded} in a particular subregion. This makes it possible for other data to inform the construction of the graph such as the connnectivity or the types of node modules to put in each node. Moreover, we can use algorithms designed for meta-learning problems to \textit{optimize} the graph itself, as we will see in subsection \ref{subsec:optimize}. Finally, GEN nodes and edges may have different node and edge neural networks, allowing dynamics to be very different in different parts of the space; for example depending on the material properties of a particular region.

Note that, in contrast with finite element methods, the dynamics of the system follow completely unknown equations; giving us a more complicated, but also more flexible, framework. In this work we take finite element methods only as inspiration to construct a general purpose method, without trying to improve upon them on their own problems; this is left for future work. 












\subsection{GEN}
A GEN consists of the following:
\begin{itemize}
    \item Embedding/hidden space $H\in \mathbb{R}^m$
    \item Graph Convolutional Network / Message Passing Neural Network
    \begin{itemize}
        \item Node module
        \item Edge module
        \item Number of message-passing steps $T$
    \end{itemize}
    \item Set of $n$ nodes $V$, each node $v_i$ has:
    \begin{itemize}
        \item States $h_t\in H$ for $t\in [0,T]$
        \item Position $p\in X$; we call $V_p$ the list of all positions.
    \end{itemize}
    \item Connectivity function $C: V_p\in X^n \rightarrow [0,1]^{n^2}$, which decides the edges as a function of the nodes positions.
    \item Set of encoder functions: $e_i: S_i \rightarrow H$
    \item Set of decoder functions: $d_i: H \rightarrow S_i$
    \item Representation function $R: x\in X \times V_p\in X^n \rightarrow \mathbb{R}^n$, expressing each position in the metric space as a function of all the nodes positions
\end{itemize}
\subsection{GEN computations}
Let $I$ be the set of inputs, triplets $(x_i,k_i, F_{k_i}(x_i))$.
$$emb_i = e_{k_i}(F_{k_i}); r_i = R(x_i)$$
$$M_R = stack(r_i); \vec{h}_0 = M'\cdot emb_i$$
$$\vec{h}_T = GCN^T(\vec{h}_0)$$
Let $Q$ be the query positions and query function $x_j, k_j$:
$r_j = R(x_j)$
$$M_r = stack(r_j); retrieval_j = M\cdot \vec{h}_T$$
$$pred_j = d_{k_j}(retrieval_j)$$
\subsection{Training data}
Training data comes from a set of tasks (like meta-learning); each with a set of function evaluation pairs $(x\in X, F_k(x))$ or $(x\in X, (q, F_k(x)(q)))$ partitioned into inputs and (query, targets).
\subsection{Objective function and training}
Minimize the sum of errors on the queries, given the GEN computations defined above. All encoders, decoders, GCN modules and potentially node positions, are trainable end-to-end.



\section{SKETCH of the framework}
\subsection{Problem class}
\iffalse
The most generic form is the following:
\begin{itemize}
    \item Metric space $X$
    \item Set of input spaces $I_1, \dots, I_{|I|}$
    \item Set of inputs, each a tuple $(x\in X, i\in I_{t_i})$
    \item Set of pairs of query spaces and output spaces $(Q_1,O_1), \dots, O_{|O|}$
    \item Set of triplets position, queries and target values: $(x\in X, q\in Q_k, t\in O_k)$
\end{itemize}
However, I think the 'query' part makes everything less clear. We can take it out (and put it back later), and now the problem class is much cleaner:
\fi
\begin{itemize}
    \item Metric space $X$.
    \item Set of stochastic functions $F_i: r\in R \rightarrow s\in S_i$.
    \item Input: set of function evaluations: $(k, x\in X, F_k(x)\in S_k)$
    \item Position, target pairs: set of evaluations  $(k, x\in X, F_k(x)\in S_k)$
    \item Target general properties
\end{itemize}
Notice that now, inputs and (position, target) pairs have the same form.

There are cases where what we want to model a function that depends on more things than just the position (for instance position and orientation). The same framework still applies, with the stochastic function being a random variable $z = (z_1\sim Z_1, z_2 \sim \hat{F}_k(x,z))$.

\textbf{Particular cases}
\begin{enumerate}
    \item When there is a single function $F$, from which both inputs and outputs come from, this looks like meta-learning.
    \item If $F_1 = f_{t=0}, F_2= f_{t=T}$ and all inputs are evaluations from $F_1$ and all outputs are evaluations from $F_2$ these correspond to the evolution of a PDE.
\end{enumerate}
